Detecting Signatures of Early-stage Dementia with Behavioural Models Derived from Sensor Data

There is a pressing need to automatically understand the state and progression of chronic neurological diseases such as dementia. The emergence of state-of-the-art sensing platforms offers unprecedented opportunities for indirect and automatic evaluation of disease state through the lens of behavioural monitoring. This paper specifically seeks to characterise behavioural signatures of mild cognitive impairment (MCI) and Alzheimer's disease (AD) in the \textit{early} stages of the disease. We introduce bespoke behavioural models and analyses of key symptoms and deploy these on a novel dataset of longitudinal sensor data from persons with MCI and AD. We present preliminary findings that show the relationship between levels of sleep quality and wandering can be subtly different between patients in the early stages of dementia and healthy cohabiting controls.

==> sections/data_acquisition_and_labelling.tex <==
% \section{Data Acquisition and Labelling} \label{data}
% \subsection{Participant Recruitment and Data Acquisition}
% Participants were primarily recruited from the cognitive disorder service at North Bristol NHS Trust and the Dementia Wellbeing Service based in Bristol. All patients with a current diagnosis of MCI or AD within the last two years may be eligible and will be selected according to the following inclusion and exclusion criteria:

% Inclusion criteria:
% \begin{itemize}
%   \item At least 50 years old
%   \item Native or fluent English speaker
%   \item Normal or corrected to normal vision
%   \item Living at home with a partner or carer
%   \item Full capacity to give informed consent
%   \item Willing to have the SPHERE system installed in their home for 12 months
% \end{itemize}

% Exclusion criteria:
% \begin{itemize}
%   \item Lives alone or in a nursing home
%   \item Study partner does not consent to the SPHERE installation
%   \item Any severe physical or psychiatric comorbidity that would interfere with their ability to take part in the study
%   \item Limited or non-English speaker
%   \item Lacks capacity to give informed consent
% \end{itemize}

% Participant behaviours will be recorded for 12 to 18 months eventually according to the project's plan. Participants will wear the SPHERE wearable on their dominant wrist. The device is equipped with two ADXL362 accelerometers, which output a continuous numerical stream of readings at $20 Hz$ (units of $g$, \ie approximately $9.81 m.s^{-2}$), and wirelessly transmits data using Bluetooth Low Energy standard to several access points installed inside different rooms of every house. Along with the accelerometer readings there is RSSI data recorded by each access point at $5 Hz$ in units of dBm, which is informative and the main basis of indoor localisation. Below is a picture of SPHERE wearable used in our study.

% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.8]{SPHERE_wearable}
% \caption{SPHERE wearable}
% \end{figure}

% \subsection{Labelling of Data}
% The location annotations were done by the technician, who carried all the wearables in a bag and walked trough every room. Inside each room he would stop for a while and make annotations, which we used as ground truth to train our classifiers.
% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.6]{annotation_example}
% \caption{An example of annotations}
% \end{figure}

==> sections/methods_old.tex <==
\section{Methods} \label{methods}

In this section we describe the machine learning pipeline used for localisation: we start by describing the data collected, the features extracted and then the machine learning model used.

\subsection{Data \& Feature Extraction}
Participants of this project were primarily recruited from the cognitive disorder service at North Bristol NHS Trust and the Dementia Wellbeing Service based in Bristol \todo{mention NHS ethics and an ID for it - RSR you got the ethics ID?}. They will wear the SPHERE wearable on their dominant wrist \cite{vafeas2020wearable,fafoutis2017designing,elsts2018guide}. The device is equipped with two ADXL362 accelerometers, which output a continuous numerical stream of readings at $20 Hz$. In every house there are $6$ gateways collecting Received Signal Strength Indicator (RSSI) data transmitted wirelessly by SPHERE wearables at 5Hz. RSSI data has range $(0, -120) dBm$ and accelerometer data correspond to multiples of the gravitational force $g$.

The labelled data is generated during a scripted data collection in each residence performed shortly after sensor deployments. The installation technician walks around the house with the wearables, passing through all the rooms, staying for a few minutes in each. Simultaneously, the real-time location of the technician is recorded, and together this makes the training data for room-level localisation.  The whole process lasts for approximately 40 minutes.

Data are extracted from the RSSI data using a window of length $5$ seconds, with an overlap of $2.50$ seconds. This is a common resolution for tasks of this form \cite{twomey2018comprehensive}. \todo{cite some SPHERE work}. 

Several challenges arise with working with this data, particularly that RSSI data suffers from missing values. There are several causes of missingness, including 1) missing at random \todo{due to what?}, and 2) unsuccessful packet delivery due to distance between gateway/wearable. \todo{Why is the data missing at random?}

To exploit the missing-due-to-distance factor we extract features, per gateway, counting the number of missing values (which is shown to be effective, even if used on its own). The features we extract from each window include (per gateway): \emph{mean}, \emph{standard deviation} (std), \emph{max}, \emph{min}, \emph{diff} (first-order difference operator) and the count of missing values.

\subsection{Model stuff}

\emph{Covariance Shift}
A further challenge we face is the difference between the training and test distributions. This contrast arises for several reasons:
\begin{itemize}
    \item Between-person walking pattern difference, which potentially gets accentuated due to the age difference.
    \item During the walk-around the wearables are kept in a backpack, while the participants are expected to be work on the wrist.
    \item During the walk-around the technician does not perform activities of daily living, e.g. prepare a cup of tea, watch TV, or lie in bed.
\end{itemize}

In mathematical terms we assume that $P_{tr}(x) \neq P_{te}(x)$, while $P_{tr}(y|x) = P_{te}(y|x)$. Given that we have no access to labelled data from the participants, we make use of the Maximum Mean Discrepancy (MMD) as presented in \cite{huang2007correcting}, which we include here for completeness. Our objective is:
\begin{equation}
    \underset{(x, y) \sim P_{te}(x, y)}{\mathbb{E}}\left[l(f_{\theta}(x), y)\right] = \underset{(x, y) \sim P_{tr}(x, y)}{\mathbb{E}}\left[\frac{P_{te}(x)}{P_{tr}(x)}\cdot l(f_{\theta}(x), y)\right]
\end{equation}
% \todo{Why does (1) hold?}
whose solution can be approximated by minimizing the weighted sample version:
\begin{equation}
    \label{eq:wsl}
    \mathcal{L}_{wsl} = 
    \sum_{(x_i, y_i) \in \hat{\mathcal{D}}_{tr}}^{N_{tr}}\frac{P_{te}(x_i)}{P_{tr}(x_i)}\cdot l(f_{\theta}(x_i), y_i) = 
    \sum_{(x_i, y_i) \in \hat{\mathcal{D}}_{tr}}^{N_{tr}}\beta_i\cdot l(f_{\theta}(x_i), y_i)
\end{equation}

The weights $\{\beta_i\}_{i=1}^{N_{tr}}$ are not known, but they can be approximated by the solution of the following convex optimization program (MMD):
\begin{align}
    \label{eq:mmd}
    &\arg \min_{\beta} \frac{1}{2} \beta^{\top} K \beta-\kappa^{\top} \beta \\
    s.t. &\beta_{i} \in[0, B] \text { and }\left|\sum_{i=1}^{N_{tr}} \beta_{i}-N_{tr}\right| \leq N_{tr}\cdot \epsilon \nonumber
\end{align}
where $\beta \in \mathbb{R}^{N_{tr}}$, $K_{ij} := k(x_i, x_j)$ and $\kappa_i := \frac{N_{tr}}{N_{te}}\cdot \sum_{j=1}^{N_{te}} k(x_i, x_j')$. $k(x_i, x_j) := \langle \psi(x_i),  \psi(x_j')\rangle$, and $\psi : \mathcal{X} \rightarrow \mathcal{F}$, maps the original input space ($\mathbb{R}^d$) to the feature space $\mathcal{F}$. In our experiments $\mathcal{F}$ is a Reproducing Kernel Hilbert Space (RKHS) generated by the Radial Basis Function (RBF).

A proof of the validity of the approximation $\beta_i \approx \frac{P_{te}(x_i)}{P_{tr}(x_i)}$ can be found in \cite{sugiyama2010density}.

For the computation of the weights in Eq.\ref{eq:mmd} we sample data uniformly at random from participant's data. The walk-around data in treated as sequential data, but rather as \emph{iid} because 1) it doesn't help with performance, and 2) the transition information\footnote{This includes, for example, between-room transition probabilities, how long you stay in each room, etc.} would be meaningless as the data is not realistic. %\todo{Clearer explanation of transition information?}

\emph{Semi-Supervised Learning}
On the other hand, in the case of participant's data, we represent them as time-series data as it is now meaningful. We use this representation both while training, in a semi-supervised fashion, and during prediction as decoding.

Conditional Random Fields (CRF) can be represented as follows:
\begin{equation}
    \label{eq:crf}
    P_{\theta'}(\boldsymbol{y} | \boldsymbol{X}) = Z(\boldsymbol{X})^{-1} \cdot \exp \left(\sum_{t=1}^{T} \phi_{t}\left(x_{t}, y_{t}, y_{t-1}\right)\right)
\end{equation}

% \todo{What is $Z(\boldsymbol{X})^{-1}$?}
(We have now shifted to considering bold-case notation to emphasize that we are dealing with high-dimensional data.)

where $\phi_t$ are the log-potentials and $Z(\boldsymbol{X})$ is the log-normaliser. In our case the log-potentials decompose, to \emph{emission} function and \emph{transition} function, as follows: $\phi_{t}\left(x_{t}, y_{t}, y_{t-1}\right)$ = $u\left(x_t, y_t\right) \cdot \tilde{\tau}(y_{t-1}, y_t)$, where: 
% \todo{Can you briefly explain these two terms -- $u\left(x_t, y_t\right) and \tilde{\tau}(y_{t-1}, y_t)$}

\begin{equation}
    \tilde{\tau}(y_t, y_{t-1}) =
    \left\{ \begin{array}{ll}
        \tau(y_t, y_{t-1}), & \alpha(t)>=\epsilon'  \\
        \mathcal{I}_{c\times c}, &\text{otherwise}
    \end{array} \right.
\end{equation}
where $\alpha(t)$ is the activity level of the participant at time $t$ and $epsilon'$ denotes a threshold, below which we assume there is no movement. The activity level $\alpha(t)$ is based on a simple computation on the accelerometer data: it is the mean of the first difference operator applied to the three axes, at time $t$.

Considering Eq.\ref{eq:wsl}, let $f_{\theta}(x) = \sigma(\boldsymbol{W}\cdot h(x))$, where $\sigma$ is the soft-max, and $h(x)$ denotes the output of a neural network. Then $u(x, y) = h(x)_y$. 

By letting $\boldsymbol{y}^* = \arg \max_{\boldsymbol{y} \in \mathcal{Y}} P(\boldsymbol{y} | \boldsymbol{X})$ then: %\todo{lack of variable for argmax?}
\begin{equation}
    \mathcal{L}_{ssl} = log  P_{\theta'}(\boldsymbol{y^*} | \boldsymbol{X})
\end{equation}

Differentiation through the \emph{arg max} operator is done by using techniques presented in \cite{alex2020torchstruct} \footnote{In our experiments we also make use of the accompanied library \emph{torch-struct} implemented in \emph{PyTorch} available at: \textrm{https://github.com/harvardnlp/pytorch-struct}.}. 

The final objective is then: $\mathcal{L} = \mathcal{L}_{wsl} + \mathcal{L}_{ssl}$.

\emph{Complementing the Labelled Data}
So far, we haven't made use of our domain knowledge beyond the sequential aspect. We can, in some cases, infer the location of the participant using our understanding of daily living. For example, people sleep at night in their bedroom, which allows us to to complement the class \emph{bedroom} with realistic data (Caution needs to be taken here as sometimes the participants do not wear the wearable.).

\emph{Model Specifics \& Optimization}
For the transformation network we used a $4$-layer neural network, with $20$ neurons per layer, and batch-normalization. For the optimization, we used \emph{ADAM} with learning rate set to $1e-2$. Implementation was carried out in \emph{PyTorch}.

\subsection{Improvements}
For the future we are looking into building along these axes:
\begin{itemize}
    \item Missing Values: Trying to differentiate the two sources is something we are looking into, with potential way being ... 
    \item Adaptive window length, possibly based on activity levels, that would allow us to have shorter windows during time of high activity levels, and longer during periods of low activity levels.
    \item Extract more realistic date from the participants, using knowledge of daily living.
\end{itemize}
